A Laboratory Experiment on Using Different Financial-Incentivization Schemes in Software-Engineering Experimentation

In software-engineering research, many empirical studies are conducted with open-source or industry developers. However, in contrast to other research communities like economics or psychology, only few experiments use financial incentives (i.e., paying money) as a strategy to motivate participants' behavior and reward their performance. The most recent version of the SIGSOFT Empirical Standards mentions payouts only for increasing participation in surveys, but not for mimicking real-world motivations and behavior in experiments. Within this article, we report a controlled experiment in which we tackled this gap by studying how different financial incentivization schemes impact developers. For this purpose, we first conducted a survey on financial incentives used in the real-world, based on which we designed three incentivization schemes: (1) a performance-dependent scheme that employees prefer, (2) a scheme that is performance-independent, and (3) a scheme that mimics open-source development. Then, using a between-subject experimental design, we explored how these three schemes impact participants' performance. Our findings indicate that the different schemes can impact participants' performance in software-engineering experiments. Due to the small sample sizes, our results are not statistically significant, but we can still observe clear tendencies. Our contributions help understand the impact of financial incentives on participants in experiments as well as real-world scenarios, guiding researchers in designing experiments and organizations in compensating developers.

==> sections/back_notused.tex <==

\section{Background and Related Work}

Experiments in software engineering are comparable to “real-effort experiments” in experimental economics, which
involve participants who solve certain tasks to increase their payoffs. Consequently, we build on experiences from
the field of experimental economics, which involves a large amount of literature on how and when to use financial
incentives in real-effort experiments [ 10, 12, 14, 39]. For instance, some findings indicate gender differences regarding
the impact of incentivization schemes, which we have to consider during our experiment. In detail, research has shown
that men choose more competitive schemes (e.g., tournaments, performance payments). Similarly, participants with
higher social preferences select such competitive schemes more rarely [9, 27]. We will consider such factors when
analyzing the results of our experiment (e.g., comparing gender differences if the number of participants allows).
Unfortunately, there is much less research on incentivization schemes in software-engineering experimentation.
Mason and Watts [26] have analyzed the impact of financial incentives on crowd performance during software projects
using online experiments. The results are similar to those in experimental economics, but the authors also acknowledge
that they did not design the incentives to mimic the real world or to improve the participants’ motivation. Other studies
have been concerned with the impact of payments on employees’ motivation [33, 37], job satisfaction [21, 36], or job
change [ 6, 13, 16]. For instance, Baddoo et al. [3] conducted a case study and found that developers perceived wages and
benefits as an important motivator, but they did not connect payments to objective performance metrics. None of the
studies we are aware of decomposes payments or wages into specific components (e.g., performance-dependent versus
performance-independent). So, the effectiveness of different payoff schemes on developers’ performance remains unclear.
Software-engineering researchers have investigated the motivations of open-source developers to a much greater
extent [11, 15, 18, 19, 43]. From the economics perspective, open-source systems represent a public good [ 5, 25 ]: they
are available to everyone and their consumption do not yield disadvantages to anyone else. A typical problem of
public goods is that individual and group incentives collide, which usually leads to an insufficient provision of the
good. While typical explanations for open-source development focus on high intrinsic motivation to contribute or
learn, this is not always the case. For instance, Roberts et al. [30] show that financial incentives can actually improve
open-source developers’ motivation (in terms of contributions). Still, financial incentives are at least not always the
predominant motivators for software developers [ 4, 33]. As a consequence, we will use the concept of open-source
software as a social good [ 19] as an extreme example (i.e., the developers help solve a social problem, but do not
receive a payment) for designing a fourth payoff function in our experiment.

==> sections/intro_notused.tex <==
\section{Introduction}

Experiments in software engineering rarely use financial incentives.
However, in the real world, software developers are compensated for their work, for instance, monetarily via wages and bug bounties~\citep{Krueger2020CommunitiesContribute,Krishnamurthy2006BugBounty} or non-monetarily via gaining reputation in open-source communities~\citep{BITZER2007160,Gerosa2021MotivationOSS}.
Economics theory and experimental practice emphasize that it can be useful to employ financial incentives in such cases to compensate experiment participants, motivate real-world behavior, and thereby improve the validity as well as realism of experiments~\citep{Weimann2019MethodsExperimentalEconomics}.
More specifically, financial incentives serve two purposes in experiments:
\begin{enumerate}
    \item they can improve the validity of an experiment by mimicking the real-world incentivization schemes to motivate realistic behavior; and

    \item they allow to study how different incentivization schemes impact participants' performance.
\end{enumerate}
For this purpose, financial incentives in economics typically involve financial rewards or penalties that are mapped onto the participants' performance.
This results in a so-called \emph{pay-off function} that describes how decisions and performance are rewarded with money, allowing to account for their actual performance and extend established show-up or participation fees.

We argue that financial incentives are also relevant within the context of software-engineering experiments, ideally improving their validity by mimicking the real world.
Interestingly, we are not aware of guidelines or recommendations on using financial incentives for software-engineering experiments.
Even the ACM SIGSOFT Empirical Standards\footnote{\url{https://github.com/acmsigsoft/EmpiricalStandards}} (September 26, 2022; commit 26815c6) did mention financial incentives only for longitudinal studies and questionnaire surveys to improve participation.
Identically, based on a literature review and our expertise in the area, financial incentives for rewarding participants’ performance during a software-engineering experiment are not
used systematically. 
Some existing studies broadly incentivize performance (e.g.,
\cite{Sayagh2020RunTimeConfigurationFramework} or \cite{Shargabi2020PerformingTasksMentalModelNovices}), but only with the idea of increasing participation.
Furthermore, we know from experimental economics~\citep{Charness2011LabLabor,Carpenter2019RealEffortTasks} that finding a realistic (and thus externally valid) way
to reward performance is challenging and no simple one-fits-all solution exists. 
For instance, the performance of
open-source developers depends less on financial rewards than those of industrial developers~\citep{Beecham2008MotivationSE,Baddoo2006MotivationDevelopers,Ye2003MotivationOpenSource,Huang2021CotntributingOSS}.

As a step towards understanding and systematizing the potential of using financial incentives in software-engineering experimentation, we~\citep{Krueger2022RegisteredReportFinancialIncentives} proposed a two-part study comprising a survey and a controlled experiment in the context of bug detection through code reviews. 
First, we conducted a survey with practitioners to elicit real-world incentivisation schemes on bug finding. 
In the survey, we distinguished between the schemes most participants prefer and those actually employed. 
Building on the results, we defined two corresponding payoff functions for our experiment.
To extend our experiment, we added two more payoff functions: one that is performance-independent and one that resembles the motives of open-source developers. 
We derived the latter function using the induced-value method established in experimental economics [35 , 42], which induces a controlled willingness of participants to achieve a desired goal (i.e., identify a bug) or obtain a certain good during an experiment by mimicking its monetary value
(e.g., a reward). 
Second, we employed our actual between-subject experiment to explore to what extent each of the four payoff functions impacts the participants’ behavior.
{\color{red}TODO}
Overall, we primarily contribute to improving researchers’ understanding that and how financial incentives can impact the outcome of software-engineering experiments. 
These results can also help to explain how different incentivisation schemes could improve practitioners’ motivation. 
Our survey and experimental design artifacts are available in a persistent open-access repository.\footnote{\url{link to Zenodo}}

==> sections/method_notused.tex <==

\section{Methodology}

As explained previously, our study involves two data-collection processes: a survey and a laboratory experiment. The experiment aims to compare pay-off functions corresponding to the following four different types of treatments: performance-independent incentives (NPIT), incentives for open-source software development (OSIT), incentives mostly preferred by practitioners (MPIT), and those mostly applied in practice (MAIT). We determine the pay-off functions for NPIT and OSIT based on established research~\cite{} and the pay-off functions for MPIT and MAIT using the data collected through the survey. 

\subsection{Survey} 
With our survey, we aim to explore \textbf{(i)} which payment components (e.g., wages only, bug bounties) are most
applied (MA) in practice and \textbf{(ii)} which payment components are most preferred (MP) by practitioners. We display an overview of these payment components with concrete examples in Table~\ref{tab:payments}. Our intention is to understand what is actually employed compared to what would be preferred as a payment schema to guide the design of our experiment.

\subsubsection{Structure} We created an online questionnaire with the structure shown in Table~\ref{tab:surveyVariables}. At first, we welcomed our participants, informing them about the survey’s topic, duration, and their right to withdraw from our experiment at any point in time without any disadvantages. Furthermore, we asked for consent to collect,
process, and publish the data anonymously. 
%To allow for questions, we will provide the contact data of at least one author on this first page. 
Then, we asked about each participant's background to collect control variables. Background information we collected comprised participants' demographics (i.e., age, gender, the country they live in, highest level of education), their role in their organization, the domain they work in, and experience with code reviews. \gc{We need to check if we managed to get a broad sample of responses. Otherwise, we need to modify the following two sentences.} These background questions allowed us to monitor whether we have acquired a broad sample of responses from different organizations and thus on varying practices. We aimed to mitigate any bias caused by external variables, such as the organizations' culture.\gc{In the registered report, we wrote that we would remove participants without code review experience. We need to check if we discarded participants with no code review experience.} Also, we discarded the answers of participants without experience with code reviews.

\gc{Should we also create a Figure that displays the survey structure as a flowchart to show the survey's adaptive nature?} Based on the participants' roles, the online survey showed the questions on the payment structures in an adaptive manner. We designed these questions as well as their answering options based on established guidelines and our experiences with empirical studies in software engineering~\cite{Siegmund2014MeasuringExperience,Nielebock2019Comments,Krueger2019Traceability}.

Following the background questions, our survey displayed the payment components (\emph{target variables}), summarized in \autoref{tab:payments} in the form of a checklist where each participant could select all components that are applied in their organization. Each selected component had a field where the participant could enter a percentage to indicate to what extent that component impacts their payment (e.g., 80\,\% wage and 20\,\% bug bounty).

We presented the same checklist and fields again to identify which subset of components the participants would prefer to contribute with what share to their payment. While the survey displayed this second list to any management role (e.g., project manager, CEO), we asked software engineers (e.g., developer, tester) to decide upon those components from the perspective of being the team or organization lead.
To prevent sequence effects, we randomized the order in which the two treatment questions (applied and preferred) occur: the survey displayed the checklist to identify the payment components applied in participants' organization and the checklist to identify those participants preferred in randomized order.  

Finally, we asked each participant to indicate how many hours per week they work unpaid overtime and used participants' responses as a type of performance penalty in the formulation of our payoff functions. We also allowed our participants to enter any additional comments on the survey.

\begin{table}[t]
	\caption{List of components of payment asked in our survey to design payoff functions for the experiment. Note that the term \emph{check} refers to participants selecting or deselecting a line of code during our experiment (i.e., marking them as buggy or correct as can be seen in \textcolor{red}{\autoref{fig:code}}).}
	\label{tab:payments}
	\centering \begin{adjustbox}{max width=\linewidth}
		\begin{tabular}{lll|rr}
			\toprule
			\textbf{payment component} & \textbf{example} & \textbf{variable} & \multicolumn{2}{c}{\textbf{survey responses}} \\
   
             & & & \textbf{applied} & \textbf{preferred} \\
			
   \midrule
			
			\multicolumn{3}{c}{\emph{not performance-based}}\\
			
            hourly wage & payment for hours spent on code review & $wage$ & 24 & 16 \\
			
            payment per task & fixed payment for conducting a code review & $payment_{fix}$ & 2 & 0 \\
			
			\midrule
			
			\multicolumn{3}{c}{\emph{performance-based}}\\
   
			reward for completing review & bonus for finding all bugs & $reward_{complete}$ & 0 & 3 \\
   
			reward for quality & bonus for correctly found bug (e.g., bug bounty) & $reward_{quality}$ & 0 & 12 \\
			
            reward for time & bonus for performing reviews fast & $reward_{time}$ & 0 & 9 \\
			
            reward for organization's performance & bonus provided based on the organization's profits & $reward_{share}$ & 12 & 16 \\
			
            penalty for low quality & penalty for mistakes within a certain period (e.g., missed bugs) & $penalty_{quality}$ & 0 & 0 \\
			
            penalty for checks & penalty for marking lines of code in the experiment & $penalty_{check}$ & \multicolumn{2}{c}{\rule[0.5ex]{3em}{0.55pt} n/a \rule[0.5ex]{3em}{0.55pt}} \\
            
			penalty for required overtime & penalty for not completing within working hours & $penalty_{time}$ & \multicolumn{2}{c}{\rule[0.5ex]{3em}{0.55pt} n/a \rule[0.5ex]{3em}{0.55pt}} \\
			
            \midrule
   
			others & specified by participants & & 1 & 1 \\

            mean overtime hours & & & 1.34 & 0.62 \\
			\bottomrule
		\end{tabular}
	\end{adjustbox}\vspace*{-2ex}
\end{table}

\subsubsection{Sampling Participants}
We invited personal contacts and collaborators from different organizations, involving software developers, project managers, and company managers. We excluded self-employed or freelancer developers as they typically ask for a fixed payment for a specific software development task or project. 
In addition, we distributed our survey through our social media networks (e.g., LinkedIn, Twitter) using a different identifier to distinguish survey responses we get from both populations.
%In addition, we distributed our survey a second version (to distinguish both populations) of our survey through our social media networks.
%We will test whether there are differences between both samples regarding our variables of interest. 
%If the MA and MP incentives are identical in both samples, we will collapse the data. 
%Otherwise, we will build on the sample of our personal contacts. 
%This allows us to have a higher level of control over the participants' software-engineering background, and their experience with code reviews.
%Our goal is to acquire at least 30 responses to obtain a reasonable understanding of applied and preferred payments.
We collected survey data from \gc{check the number of participants} \textcolor{red}{\hl{X}} participants. As we did not evaluate the survey data using inferential statistics, we could base our sample-size planning on the limited access to a small, specialized number of participants. \gc{Is there any rationale behind not paying the survey participants? We should also discuss in the paper in relation to threats to validity of our research study.} Furthermore, we did not pay incentives to any survey participant. 

\subsubsection{Pilot}
We conducted a pilot study with \gc{check the number of participants} \textcolor{red}{\hl{three}} participants, who are Ph.D. students from our work groups, to verify the required time and understandability of the survey. Pilot results confirmed that the survey does not take more than 10 minutes.  

\begin{table}[!b]
	\caption{List of variables we will checked in our survey.}
	\label{tab:surveyVariables}
	\centering \begin{adjustbox}{max width=\linewidth}
		\begin{tabular}{lll}
			\toprule
			\textbf{variable} & \textbf{description} & \textbf{operationalization}\\
			
			\midrule
			
			\multicolumn{3}{c}{\emph{control variables}}\\
			
			demographics & age, gender, living country, highest level of education &  nominal (single-choice list)\\
			role & participant's role in their organization & nominal (single-choice list)\\
			experience & years of experience in software development and code reviewing & 6-level Likert scale ($<$1 -- $>$15)\\
			frequency & current involvement in software development and code reviewing & 5-level Likert scale (none at all -- daily)\\
			domain & domain of the participant's organization & nominal (single-choice list)\\
			size of organization & number of employees & 5-level Likert scale ($<$21 -- $>$200)\\
			size of team & number of members in participant's team (if applicable) & 6-level Likert scale (1 -- $>$50)\\
			development process & whether agile or traditional development processes are employed & $\circ$ agile $\circ$ non-agile \\
			
			\midrule
			
			\multicolumn{3}{c}{\emph{target variables}}\\
			MA/MP incentives & list of payment components that can be selected (cf. \autoref{tab:payments}) & nominal (checklist)\\ 
			MA/MP percentage & percentage to weigh the payment components chosen before & continuous (0--100\,\%)\\
			working hours per week & weekly working hours according to the participant's contract & continuous\\
			unpaid overtime & potential unpaid overtime of employees in proportion to working hours per week & ratio\\
			
			\bottomrule
			\multicolumn{3}{c}{MA: most applied; MP: most preferred}
		\end{tabular}
	\end{adjustbox}\vspace*{-2ex}
\end{table}

\subsubsection{Eliciting the Pay-Off Functions} To specify the payoff functions for our experiment, we considered the absolute frequency of combinations of different payment components.
Precisely, to identify each of the MA and MP combinations, we chose the respective combination that was selected by the largest number of respondents (i.e., modal value) and computed the mean values for the weights of each component in that combination. For instance, assume that most of our participants (e.g., $N$ participants) would state to prefer the combination of fixed wages and bug bounties. Then the pay-off function for MPIT would be $w_1 * payment_{fix} + w_2*(bugs_{correct} * reward_{quality})$, where $w_1 = (\sum_{i=1}^{N} w_{1,i})/N$ and $w_2 = (\sum_{i=1}^{N} w_{2,i})/N$  ($w_{1,i}$ and $w_{2,i}$ would be the percentages that the $i^{th}$ participant entered to indicate the extent fixed wages and bug bounties impact their payment). \gc{Rather than giving a hypothetical example should we write here the resulting pay-off functions for MAIT and MPIT?} Assume that $w_{1,i} = 75\ \%$ and $w_{2,i} = 25\ \%$, then we would define a pay-off function as $0.75 * payment_{fix} + 0.25*(bugs_{correct} * reward_{quality})$. 
Before calculating the component weights in the pay-off functions for MA and MP, we performed a graphical-outlier analysis using boxplots~\cite{tukey1977exploratory}, excluding participants with extreme values (i.e., three inter quartile ranges above the third quartile or below the first quartile).
%As an example, assume that most of our participants would state to prefer the combination of fixed wages (with a weight of 75\,\% on average) and bug bounties (25\,\% on average). Then, we would define a cost function as $0.75 * payment_{fix} + 0.25*(bugs_{correct} * reward_{quality})$.

\subsection{Laboratory Experiment}
After eliciting which payoff functions are used and preferred in practice, we conducted a laboratory experiment to measure the impact of different payoff functions in software engineering experiments. We focused on code reviews and bug identification in this experiment, since these are typical tasks in software engineering that also involve different
types of incentives. In this section, we explain the design of our experiment.

\subsubsection{Hypotheses}
We aim to support software engineering researchers by identifying which payoff functions can be used to improve the validity of experiments. Therefore, we firstly investigated the effect of performance-based incentivisation (i.e., OSIT, MAIT, MPIT) compared to incentivisation that is not performance-based (i.e., NPIT). We hypothesized that performance-based incentivisation (i.e., OSIT, MAIT, MPIT) leads to a better performance compared to incentivisation that is \textit{not} performance-based (i.e., NPIT).

\begin{center}
	\begin{rqbox}
		\begin{description}
			\item[$H0_1$:]Participants without performance-based incentivization (NPIT) have on average a worse performance than those with performance-based incentivization (e.g., OSIT, MAIT, MPIT).
		\end{description}
	\end{rqbox}
\end{center}
To investigate which performance-based incentivisation leads to a better performance, we further hypothesized that participants' experimental performance differs depending on how the performance-based incentivisation is defined. 

\begin{center}
	\begin{rqbox}
		\begin{description}
			\item[$H0_2$:]The experimental performance of participants under performance-based incentivization (e.g., OSIT, MAIT, MPIT) differs between treatments.
		\end{description}
	\end{rqbox}
\end{center}

Besides analyzing these hypotheses, we compared the behavior (e.g. risk taking) and performance between all groups to understand which incentives have what impact. Moreover, we used eye trackers to explore fixation counts, fixation lengths, and return fixations. This allowed us to obtain a deeper understanding of the search and evaluation processes during code reviews. Also, it enabled us to investigate potential differences in eye movements depending on the incentivization. More precisely, we intended to follow similar studies from software engineering~\cite{Abid2019DevelopersReadingBehavior} to explore how our participants read the source code, for instance, did they focus on the actually buggy code, what lines were they reading more often, or which code elements did they focus on to explore bugs? We reported all findings from the eye-tracking data as exploratory outcomes. The eye-tracking data was preprocessed by the firmware of Tobii (Version 1.181.37603) using the Tobii I-VT (fixation) filter.

\subsubsection{Experiment Design and Structure}
Initially, we aimed to employ a 4x1 between-subject design, where for each treatment (i.e., NPIT, OSIT, MAIT, MPIT), we would only change the payoff function. As our survey results indicated no differences between the pay-off functions for MAIT and MPIT, we combined these two treatments. Hence, our experiment ended up being a 3 x 1 between-subject design. We allocated the participants randomly to one of the three treatments, without anyone repeating the experiment in another treatment. We executed the experiment at the experimental laboratory MaXLab of the Otto-von-Guericke University using a standardized experimental environment. We measured all participants’ performance and the eye movement of four participants (restricted by number of devices) \gc{I should ask this to \hl{Dmitri}: Should we write ``in each treatment" here? Does each session correspond to a single treatment?} \textcolor{red}{\hl{in each session}} using eye trackers (60 Hz Tobii Pro Nano H). Eye trackers were mounted to the screen and barely noticeable (i.e., not a helmet the participants have to wear). Hence, eye trackers were not likely to have any impact. Yet, we also investigated possible impact wearing eye-trackers may have on our participants during our analysis. In the following subsections, we explain the procedure for each session.

\begin{enumerate}
\item \textbf{Welcome and Experimental Instructions:} After the participants of a session entered the laboratory, they were randomly allocated to working stations with the experimental environment installed. Moreover, four of the participants were randomly selected for using eye trackers. \gc{Ask \hl{Dmitri} if this was the case during the experiment, i.e., some students refused to wear eye trackers. If not, we may need to exclude the following sentences. Also, we might want to move this sentence to the ``Threats to Validity" section.} \textcolor{red} {In our invitation for the experiment we stated that the participants could be asked to use eye-trackers involved in the experiment. If a participant nonetheless disagreed to participate using eye trackers, we excluded them from the experiment to avoid selection bias.} The experimenter started each session once the participants of that session were at their places. The participants initially received general information about the experiment (e.g., welcoming text), information about the task at hand (code review), explanation on how to enter data (e.g., check box), and the definition of their payoff function for the experiment (with some examples).
\item \textbf{Review Task:} All participants received the code example with the task to identify any bugs within it (Figure~\ref{fig:code}). We did not inform the participants about the precise number of bugs in the code. Instead, a message explained that the code did not behave as expected when it was executed. At the end of the task, we can incorporate unpaid overtime as a payment component by asking participants to stay for five more minutes to work on the task.
\item \textbf{Post-Experimental Questionnaire:} After the experiment, we asked our participants a number of demographic questions (i.e., gender, age, study program, study term, programming experience). Following demographic questions, we further applied the distress sub-scale of the Short Stress State Questionnaire~\cite{helton2004validation} to measure arousal and stress of the participants. Eliciting such data on demographics and arousal enabled us to identify potential confounding parameters.

\item \textbf{Payoff Procedure:} After having collected all the data, we provided the participants information about their performance and
payoff to the participants by displaying them on their screen. We paid out these earnings privately in a separate room in cash immediately afterwards.
\end{enumerate}

\subsubsection{Code Example}
 The subject system used in the experiment is a sorting and searching Java code example that we selected and adapted from the ``The Algorithms" GitHub repository. In Figure~\ref{fig:code}, we display a screenshot of the sorting and searching code example as we will show it to participants in the lab. We selected this code example since it is: \textbf{(i)} written in Java, one of the most popular programming languages~\cite{TIOBE-index}; \textbf{(ii)} suitable for the injection of bugs; \textbf{(iii)} self-contained; \textbf{(iv)} feasible for the participants comprising students and faculty members of the Faculty for Computer Science of the Otto-von-Guericke University Magdeburg, Germany. 

 \begin{figure}[h]
    \centering
    \caption{Screenshot of the code example we used.}
    \includegraphics[width=0.9\linewidth]{graphics/CodeReview.png}
    \label{fig:code}
\end{figure}
 
 We initially selected and adapted three different Java code examples including a limited calculator from the learning platform LeetCode and a Stack example from the “The Algorithms” GitHub repository in addition to the sorting and searching example. To create buggy examples, we injected three bugs into each code example by using mutation operators [20]. Note that we partly reworked the examples to make them more suitable for our experiment (e.g.,
combining searching and sorting), added comments at the top of each example explaining its general purpose, and
kept other comments (potentially adapted) as well as identifier names to improve the realism. We aimed to limit the
time of the experiment to avoid fatigue and actually allow for a laboratory setting, and thus decided to use only one
example. To select the most suitable subject system for our experiment, we performed a pilot study in which we
measured the time and performance of the participants. In detail, we asked one M.Sc. student from the University of
Glasgow who has worked as a software practitioner in industry and four PhD students from the University of Zurich to
perform the code reviews on the buggy examples. Overall, each example was reviewed by three of these participants.
Our results indicate that the sorting and searching example would be most feasible (i.e., $\approx$12 min, 4/9 bugs correctly
identified, 5 false positives), considering that the task should neither be too easy nor to hard, the background of the
pilot’s participants and the potential participants for our experiment, as well as the examples’ quality. The other
two examples seemed too large or complicated (i.e., $\approx$14 min, 2/9 bugs; 4 false positives; $\approx$8 min, 5/9 bugs, 8 false
positives), which is why we decided to use the sorting and searching example (available in our artifacts). We remark
that none of the participants from this pilot study will be involved in our actual experiment. 





